Properties and Complexity of Fan-Planarity

In a \emph{fan-planar drawing} of a graph an edge can cross only edges with a common end-vertex. Fan-planar drawings have been recently introduced by Kaufmann and Ueckerdt, who proved that every $n$-vertex fan-planar drawing has at most $5n-10$ edges, and that this bound is tight for $n \geq 20$. We extend their result, both from the combinatorial and the algorithmic point of view. We prove tight bounds on the density of constrained versions of fan-planar drawings and study the relationship between fan-planarity and $k$-planarity. Furthermore, we prove that deciding whether a graph admits a fan-planar drawing in the variable embedding setting is NP-complete.

==> bipartite.tex <==
\section{Density of $2$-layer Fan-planar Graphs}\label{se:bipartite}

We already observed that a $2$-layer fan planar graph $G$ is an outer fan-planar graph. Also, since all vertices on the same layer form an independent set, graph $G$ is bipartite. We prove the following.

\begin{theorem}\label{th:2layer}
A $2$-layer fan-planar graph with $n$ vertices has at most $2n-4$ edges, and this bound is tight for $n \geq 3$.
\end{theorem}
\begin{proof}
Let $G$ be a maximally dense $2$-layer fan-planar graph with $n$ vertices and $m$ edges, and let $\Gamma$ be a $2$-layer fan-planar drawing of $G$. Denote by $V_1=\{v_1,\dots,v_{n_1}\}$ and $V_2=\{v_{n_1+1},\dots,v_{n}\}$ the two independent sets of vertices of $G$. Without loss of generality, suppose that in $\Gamma$ we have $v_i$ precedes $v_{i+1}$ along the layer of $V_1$ (for $i=1,\dots,n_1-1$), and $v_j$ precedes $v_{j+1}$ along the layer of $V_2$ (for $j=n_1+1,\dots,n-1$). See Figure~\ref{fi:2layer-proof}. Construct from $G$ a super-graph $G^*$, by adding an edge $(v_i,v_{i+1})$, for $i=1,\dots,n_1-1$, and an edge $(v_j,v_{j+1})$, for $j=n_1+1,\dots,n$ (see Figure~\ref{fi:2layer-proof-2}). Graph $G^*$ is still outer fan-planar. Moreover, $G$ does not contain a $K_5$ subgraph (because $G$ is bipartite), and this implies that also $G^*$ does not contain a $K_5$ subgraph, as otherwise at least three vertices of the same layer in $G$ should form a $3$-cycle in $G^*$ (which does not happen by construction). Thus, by Lemma~\ref{le:oddcycles} and Property~\ref{pr:3-mutually}, the crossing graph of any outer fan-planar drawing of $G^*$ contains only even cycles. Hence, denoted as $m^*$ the number of edges of $G^*$, by Lemma~\ref{le:3n-6} we have $m^* \leq 3n-6$, and therefore $m = m^* -(n-2) \leq 2n-4$.

\begin{figure}
\centering
\subfigure[]{\includegraphics[width=0.32\columnwidth]{figures/2layer-proof}\label{fi:2layer-proof}}\hfill
\subfigure[]{\includegraphics[width=0.32\columnwidth]{figures/2layer-proof-2}\label{fi:2layer-proof-2}}\hfill
\subfigure[]{\includegraphics[width=0.32\columnwidth]{figures/2layer-maximallydense}\label{fi:2layer-maximallydense}}
\caption{Illustration of the proof of Theorem~\ref{th:2layer}.}\label{fi:2layer}
\end{figure}

A family of $2$-layer fan-planar graphs with $2n-4$ edges is the family of the bipartite complete graphs $K_{2,n-2}$ (see Figure~\ref{fi:2layer-maximallydense}).\qed
\end{proof}

\remove{
\begin{corollary}\label{co:bipartite}
Every maximally dense $2$-layer fan-planar graph with $n \geq 3$ vertices has $2n-4$ edges.
\end{corollary}
}%end remove
